GeneFace++: Generalized and Stable Real-Time Audio-Driven 3D Talking Face Generation

Generating talking person portraits with arbitrary speech audio is a crucial problem in the field of digital human and metaverse. A modern talking face generation method is expected to achieve the goals of generalized audio-lip synchronization, good video quality, and high system efficiency. Recently, neural radiance field (NeRF) has become a popular rendering technique in this field since it could achieve high-fidelity and 3D-consistent talking face generation with a few-minute-long training video. However, there still exist several challenges for NeRF-based methods: 1) as for the lip synchronization, it is hard to generate a long facial motion sequence of high temporal consistency and audio-lip accuracy; 2) as for the video quality, due to the limited data used to train the renderer, it is vulnerable to out-of-domain input condition and produce bad rendering results occasionally; 3) as for the system efficiency, the slow training and inference speed of the vanilla NeRF severely obstruct its usage in real-world applications. In this paper, we propose GeneFace++ to handle these challenges by 1) utilizing the pitch contour as an auxiliary feature and introducing a temporal loss in the facial motion prediction process; 2) proposing a landmark locally linear embedding method to regulate the outliers in the predicted motion sequence to avoid robustness issues; 3) designing a computationally efficient NeRF-based motion-to-video renderer to achieves fast training and real-time inference. With these settings, GeneFace++ becomes the first NeRF-based method that achieves stable and real-time talking face generation with generalized audio-lip synchronization. Extensive experiments show that our method outperforms state-of-the-art baselines in terms of subjective and objective evaluation. Video samples are available at https://genefaceplusplus.github.io .

==> sections/5_related.tex <==
\section{Related works}

\subsection{Text-to-Speech}
Text-to-speech (TTS) models convert input text or phoneme sequence into mel-spectrogram (e.g., Tacotron~\cite{wang2017tacotron}, FastSpeech~\cite{ren2019fastspeech}), which is then transformed to waveform using a separately trained vocoder~\cite{kong2020hifi,huang2021multi}, or directly generate waveform from text (e.g., EATS~\cite{donahue2020end} and VITS~\cite{kim2021conditional}). Early autoregressive models~\cite{wang2017tacotron,li2019neural} sequential generate a sample and suffer from slow inference speed. Several works~\cite{ren2019fastspeech,kim2020glow} have been proposed to generate mel-spectrogram frames in parallel, which speed up mel-spectrogram generation over autoregressive TTS models, while preserving the quality of synthesized speech. Recently proposed Diff-TTS~\cite{jeong2021diff}, Grad-TTS~\cite{popov2021grad}, and DiffSpeech~\cite{liu2021diffsinger} inherently are gradient-based models with score matching objectives to generate high-quality samples, while the iterative sampling process costs hinder their applications to text-to-speech deployment. Unlike the dominant gradient-based TTS models mentioned above, ProDiff directly predicts clean data and frees from estimating the gradient for score matching. The proposed model avoids significant perceptual quality degradation when reducing reverse iterations, and thus it maintains sample quality competitive with state-of-the-art models using hundreds of steps. 

\subsection{Diffusion Probabilistic Models}
Denoising diffusion probabilistic models (DDPMs)~\cite{ho2020denoising,song2020denoising,lam2021bilateral} are likelihood-based generative models that have recently succeeded to advance the state-of-the-art results in several important domains including image synthesis~\cite{dhariwal2021diffusion,song2020denoising}, audio synthesis~\cite{huang2022fastdiff}, and 3D point cloud generation~\cite{luo2021diffusion}, and have proved its capability to produce high-quality samples. One major drawback of diffusion or score-based models is the slow sampling speed due to many iterative steps. To alleviate this issue, multiple methods have been proposed, including learning an adaptive noise schedule~\cite{lam2022bddm}, introducing non-Markovian diffusion processes~\cite{song2020denoising}, and using adversarial learning for reducing iterations~\cite{xiao2021tackling}. To conclude, all these methods focus on the image domain, while audio data is different for its long-term dependencies and strong condition. ~\citet{liu2022diffgan} proposes a denoising diffusion generative adversarial networks (GANs) to achieve high-fidelity and efficient text-to-spectrogram synthesis. Differently, our work focuses on designing progressive fast diffusion models for text-to-speech synthesis without unstable adversarial learning procedure, which has been relatively overlooked.

\subsection{Knowledge distillation}
Knowledge distillation has been demonstrated for its efficiency in simplifying the data distribution. In non-autoregressive machine translation~\cite{gu2017non}, sequence-level knowledge distillation~\cite{kim2016sequence} has achieved good performance in transferring the knowledge from the teacher model to the student. In non-autoregressive text-to-speech synthesis~\cite{ren2019fastspeech}, researchers alleviate the one-to-many mapping problem by using the generated mel-spectrogram from an autoregressive teacher model as the training target. Recently, ~\citet{salimans2022progressive} utilize knowledge distillation and iteratively halve the diffusion steps of the continuous diffusion model, accelerating iterative refinement to a large extent. In contrast, ProDiff with discrete schedules adopts knowledge distillation to reduce data variance and promote training convergence. 

==> sections/old.tex <==
\subsection{Adversarial learning}

In ProDiff, we parameterize the denoising model by $p_\theta(\vx_{t-1}|\vx_t) := q(\vx_{t-1}|\vx_t,\vx_0=f_{\theta}(\vx_t|t,c))$. Since conditional GANs with adversarial learning~\cite{yang2021ganspeech,min2021meta} have been shown to model complex conditional distributions in speech synthesis, we adopt them to approximate the true denoising distribution $q\left(\vx_{t-1}|\vx_{t}\right)$. Our training is formulated by matching the conditional GAN generator $p_{\theta}(\vx_{t-1}|\vx_{t})$ and $q(\vx_{t-1}|\vx_{t})$ using an adversarial loss that minimizes a divergence $D_{\mathrm{adv}}$ per denoising step:

\begin{equation}
    \min _{\theta} \sum_{t \geq 1} \mathbb{E}_{q(t)}[D_{\mathrm{adv}}(q(\vx_{t-1}|\vx_{t}) \| p_{\theta}(\vx_{t-1}|\vx_{t}))]
\end{equation}

where $D_{\mathrm{adv}}$ can be Wasserstein distance, Jenson-Shannon divergence, or f-divergence depending on the adversarial training setup. 

To set up the adversarial training, we denote the conditional time-dependent discriminator as $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c)$ with parameters $\phi$. It takes the N-dimensional $\vx_{t-1}$ and $\vx_{t}$ as inputs, and decides whether $\vx_{t-1}$ is a plausible denoised version of $\vx_{t}$ conditioned on intermediate features $c$. We use the least-squares loss~\cite{mao2017least} for adversarial training:
\begin{align} ~\label{eq: discriminator}
    \begin{split}
    \min _{\phi} \sum_{t \geq 1} \mathbb{E}_{q(\vx_{t})}[\mathbb{E}_{q(\vx_{t-1}|\vx_{t})}[(D_{\phi}(\vx_{t-1}, \vx_{t}, t, c) - 1)^2] \\+\mathbb{E}_{p_{\theta}(\vx_{t-1}|\vx_{t})}[D_{\phi}(\vx_{t-1}, \vx_{t}, t, c)^2],
\end{split}
\end{align}

where fake samples from $p_{\theta}(\vx_{t-1}|\vx_{t})$ are contrasted against real samples from $q(\vx_{t-1}|\vx_{t})$.

Given the discriminator, we updates the generator with following GAN objective:
\begin{equation} \label{eq: generator}
\min _{\theta} \sum_{t>1} \mathbb{E}_{q(\vx_{t})} \mathbb{E}_{p_{\theta}(\vx_{t-1}|\vx_{t})}[(D_{\phi}(\vx_{t-1}, \vx_{t}, t, c) - 1)^2]
\end{equation}


\subsection{Motivation}
Previous diffusion models~\cite{jeong2021diff,liu2021diffsinger} mainly utilize the simple loss objective (e.g., MSE or MAE) to reconstruct acoustic features. However, this optimization is demonstrated~\cite{ren2022revisiting,liu2021diffsinger} to be based on the incorrect unimodal distribution assumptions, leading to blurry and oversmoothing predictions in mel-spectrograms.

2) ProDiff adopts the adversarial training method to prevent the over-smooth issues in generated samples. Generative adversarial networks~\cite{goodfellow2014generative} with competitive games assist to model the dependent and multimodal distribution~\cite{ren2022revisiting,yang2021ganspeech}, which equip ProDiff with ablity to generate samples of high perceptual quality.


\subsection{Architecture}
4) adversarial loss $\gL_{adv}$: the GAN objectives with conditional time-dependent discriminators to minimize a divergence $D_{\mathrm{adv}}$ per denoising step; 


The spectrogram discriminator, $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c=\text{mel})$, takes ground-truth mel spectrograms as input, and measure the similarity of distribution between generated and real acoustic features as well as consider whether the generated samples match the input spectrogram. It adopts multiple random window discriminators (MWRDs)~\cite{wu2020adversarially} with random window sizes which are independent of each other. In addition, the random window sizes in MRWDs have been demonstrated for its efficiency in reducing the computational complexity in training.

The phoneme discriminator, $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c=\text{phoneme})$, takes phoneme sequences as input, and distinguishes the real speech from the generated speech given the phoneme sequence tq as the condition. In particular, the phoneme discriminator consists of fully-connected layers and is applied at frame level. Since we know the duration of each phoneme, we can concatenate each frame in mel-spectrogram with the corresponding phoneme. The discriminator then computes scalars for each frame and averages them to get a single scalar.

\subsection{Related work}

\subsection{Adversarial learning}
Adversarial learning has showed powerful performance in several image domains~\cite{wang2018high,zhang2018stackgan++}, and is adopted successfully in speech domain. GAN-based neural vocoders~\cite{kong2020hifi,kumar2019melgan} show comparable performance to the autoregressive state-of-the-art model and can synthesize speech in real-time. Researchers~\cite{donahue2020end} found that an important advantage of adversarial losses for TTS is a focus on realism over diversity, which enables a more efficient use of capacity compared to models trained with maximum likelihood. Different from previous work, we adopts the adversarial training method to prevent the over-smooth issues in generated samples.
